People on Media: Jointly Identifying Credible News and Trustworthy Citizen Journalists in Online Communities

Media seems to have become more partisan, often providing a biased coverage of news catering to the interest of specific groups. It is therefore essential to identify credible information content that provides an objective narrative of an event. News communities such as digg, reddit, or newstrust offer recommendations, reviews, quality ratings, and further insights on journalistic works. However, there is a complex interaction between different factors in such online communities: fairness and style of reporting, language clarity and objectivity, topical perspectives (like political viewpoint), expertise and bias of community members, and more. This paper presents a model to systematically analyze the different interactions in a news community between users, news, and sources. We develop a probabilistic graphical model that leverages this joint interaction to identify 1) highly credible news articles, 2) trustworthy news sources, and 3) expert users who perform the role of "citizen journalists" in the community. Our method extends CRF models to incorporate real-valued ratings, as some communities have very fine-grained scales that cannot be easily discretized without losing information. To the best of our knowledge, this paper is the first full-fledged analysis of credibility, trust, and expertise in news communities.

==> findings.tex <==

\section{Findings}

==> hypotheses.tex <==


\section{Hypotheses Testing}
\label{sec:hypotheses}

In order to validate all the hypotheses presented in Section~\ref{sec:newscom} we perform some preliminary experiments using the {\em ground-truth} article ratings in {\em newstrust.net}.

\noindent{\bf Writing Style}: We consider five qualitative indicators of writing style in the NewsTrust community, and its effect on the overall article credibility rating for stories that have atleast $3$ reviews. Table~\ref{tab:langFactors} shows Pearson's product-moment correlation of the individual aspect ratings with the overall article credibility rating. All reported results are statistically significant (with {\em P-value} $2e-16$).

\begin{table}
\centering
\small
 \begin{tabular}{p{1.7cm}p{5cm}p{1cm}}
 \toprule
 \textbf{Aspects} & \textbf{Description} & \textbf{Corr.}\\\midrule
  Insightful & Is it well reasoned? thoughtful? & 0.77\\
  Fairness & Is it impartial? or biased? & 0.75\\
  Style & Is this story clear? concise? compelling? well-written? & 0.65\\
  Responsibility & Are claims valid, ethical, unbiased? & 0.72\\
  Balance & Does this story represent diverse viewpoints? & 0.49\\\bottomrule
 \end{tabular}
 \caption{Pearson's product-moment correlation of different qualitative indicators of {\em writing style} with the overall article credibility rating (with {\em P-value} $2e-16$ for each test).}
 \label{tab:langFactors}
\end{table}

NewsTrust also captures the correctness of information provided in the news article by different indicators. Although we do not deal with them in this work --- which require a background knowledge-base for computation --- we show their effect on the overall article credibility rating in Table~\ref{tab:facts}.

\begin{table}
\centering
\small
 \begin{tabular}{p{3cm}p{1cm}p{3cm}p{1cm}}
  \toprule
 \textbf{Aspects} & \textbf{Corr.} & \textbf{Aspects} & \textbf{Corr.}\\\midrule
informative (new information) & 0.80 & enterprise (initiative, courage) & 0.64\\
sourcing (multiple sources) & 0.72 & originality (new perspective) & 0.62\\
in-depth(well-researched) & 0.70 & accurate (truthful) & 0.59\\
relevance (newsworthy, meaningful) & 0.65 & expertise (citing experts) & 0.52\\
facts (factual) & 0.64 & transparent (enough links and references) & 0.44\\\bottomrule
\end{tabular}
 \caption{Pearson's product-moment correlation of factual indicators of news with the overall article credibility rating (with {\em P-value} $2e-16$ for each test).}
 \label{tab:facts}
\end{table}

\noindent{\bf Influence of Politics}: We perform Pearson's product-moment correlation test on the standard deviation of credibility rating of an article $a$ by different members, and the influence of {\em Politics} in the news content given by $\text{Association}(a, \text{``Politics''})$ (refer to Equation~\ref{XXX}). A positive correlation of $0.11$ (with {\em P-value} $2.2e-16$) indicates a weak trend of disagreement increasing with the increase in political content of news.

\noindent{\bf User Engagement}: We ran a linear regression model using the {overall\em ground-truth} user expertise as the response variable with features of user engagement like answers, ratings given, comments, ratings received, disagreement and number of raters. The features are found to be statistically significant with {\em P-value} < $0.0001$.

\noindent{\bf Expertise Vs. Agreement}: In order to measure user disagreement, we take the mean absolute deviation of a user's rating from the community mean rating over all the stories having atleast $3$ reviews. In the above regression experiment, the model learns a negative weight for the disagreement feature (i.e. positive agreement) for predicting user expertise.
We use Pearson's product-moment correlation test to find out the correlation between user disagreement and expertise in the community. There is an overall correlation of $-0.10$ (with \textit{P-value} $1.6e-11$) between user expertise, and his disagreement with other community members. A negative sign of correlation shows a weak trend of decrease in disagreement with increase in expertise.
The effect is more pronounced for highly expert members (member level $\in [4, 5]$), with a moderate correlation of $-0.31$ (with \textit{P-value} $0.003$), who show more agreement on credibility rating of articles.

\noindent{\bf User User Interaction}: We use Pearson's product-moment correlation test to find out the correlation between the ratings received by a user from other users (on his article ratings), and his expertise in the community. There is a moderate correlation of $0.40$ (with \textit{P-value} $2.2e-16$) between user expertise, and the feedback from the community on his ratings.

\noindent{\bf Source Article Interaction}: We use Pearson's product-moment correlation test to find out the correlation between \textit{trustworthiness} of the sources and \textit{credibility} of the articles generated by them. Trustworthy sources generate credible articles having a moderate correlation of $0.47$ (with \textit{P-value} $2.2e-16$) between the two. %The $95\%$ confidence interval is $[ 0.44,\ 0.49]$.

\noindent{\bf User Article Interaction}: We use Pearson's product-moment correlation test to find out correlation between the error committed by a user in identifying credible articles, and his expertise in community. There is a negative correlation of $-0.29$ (with \textit{P-value} $2.2e-16$) indicating a weak tend of the error in credibility judgment of a user decreasing with increase in his expertise. As trustworthy sources generate credible articles and expert users can reliably identify them, the \textit{user source} interaction can be captured from above interactions.

==> objectives.tex <==
We specifically address the following issues:
\squishlisttwo
\item How does the {\em writing style} of news article affect the credibility of news?
%The news articles are generally written in a polished and sophisticated language. Although it is easy for the linguists to identify the subtle linguist elements in the article~\cite{???}, do they play any significant role in the mind of ordinary readers that influence their judgment on the credibility of the articles?
\item What is the role of the underlying {\em topic} distribution of news in its credibility rating by the people?
\item How do the various traits of {\em news source} like the type of media, format of news, political viewpoint and expertise influence its trustworthiness?
\item What are the indicators of {\em user expertise} in identifying credible articles in a news community?
%\item Since credibility is subjective, can there be any agreement between the users on an article's credibility?
\item How can we model the {\em joint interaction}  between \emph{credibility} of news, \textit{objectivity} of language, \emph{trustworthiness} of media sources and \emph{expertise} of users in a news community? %What are the kinds of bias operating within?
\item How can we use such a model to identify credible articles, trustworthy sources, and expert users on specific topics?
\squishend
